Novel methods for multilinear data completion and de-noising based on tensor-SVD

In this paper we propose novel methods for completion (from limited samples) and de-noising of multilinear (tensor) data and as an application consider 3-D and 4- D (color) video data completion and de-noising. We exploit the recently proposed tensor-Singular Value Decomposition (t-SVD)[11]. Based on t-SVD, the notion of multilinear rank and a related tensor nuclear norm was proposed in [11] to characterize informational and structural complexity of multilinear data. We first show that videos with linear camera motion can be represented more efficiently using t-SVD compared to the approaches based on vectorizing or flattening of the tensors. Since efficiency in representation implies efficiency in recovery, we outline a tensor nuclear norm penalized algorithm for video completion from missing entries. Application of the proposed algorithm for video recovery from missing entries is shown to yield a superior performance over existing methods. We also consider the problem of tensor robust Principal Component Analysis (PCA) for de-noising 3-D video data from sparse random corruptions. We show superior performance of our method compared to the matrix robust PCA adapted to this setting as proposed in [4].

==> PerformanceEvaluation.tex <==
%\vspace{-2mm} 
\subsection{Performance evaluation of video data completion}
%\vspace{-2mm} 
%\input{PerformanceEvaluation_Jamie}
In this part we test 3 algorithms for video data completion from randomly missing entries:  TNN minimization of Section \ref{sec:tcompletion}, Low Rank Tensor Completion (LRTC) algorithm in \cite{Ji_PAMI12}, which uses the notion of tensor-n-rank \cite{GandyRY2011}, and the nuclear norm minimization on the vectorized video data using the algorithm in \cite{Cai_SVT}. As an application of the t-SVD to higher order tensor we also show performance on a 4-D color Basketball video data of size $144 \times 256 \times 3 \times 80$. 
%It is a 4th order tensor and we can use tSVD to decompose this tensor then get the recovery similarly using LRTC and tensor-nuclear-norm minimization. 

Figures ~\ref{fig:recovery} and \ref{fig:basketball_color} show the results of recovery using the 3 algorithms. Figure~\ref{fig:recovery_rse} shows the RSE (dB) plots for sampling rates ranging from $10\%$ to $90\%$ where the sampling rate is defined to be the percentage of pixels which are known. Results from the figures show that the TNN minimization algorithm gives excellent reconstruction over the LRTC and Nuclear norm minimization.  These results are in line with the compressibility results in Section~\ref{sec:compression}.

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c c }
      \includegraphics[width = .14\textwidth]{figs/recovery_figs/basketball_color_10_sample.png}  \hspace{2mm}
      \includegraphics[width = .14\textwidth]{figs/recovery_figs/basketball_color_10_LRTC.png}     \hspace{2mm}
      \includegraphics[width = .14\textwidth]{figs/recovery_figs/basketball_color_10_TNN.png} \\
      \end{tabular}}
  \caption{ Recovery for color basketball video: \textbf{Left}: Sampled Video($10\%$). \textbf{Middle}: LRTC recovery. \textbf{Right}: Tensor-nuclear-norm minimization recovery }
\label{fig:basketball_color}
\end{figure}    

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c }
    \includegraphics[width = .25\textwidth]{figs/merl_error.png} 
    \includegraphics[width = .25\textwidth]{figs/basketball_error.png}
    \end{tabular}}
  \caption{ RSE (dB) plot against sampling rate \textbf{Left}: MERL video. \textbf{Right}: Basketball video }
\label{fig:recovery_rse}
\end{figure}    



==> ProblemSetUp.tex <==
\section{Tensor completion/prediction from missing observations}
\vspace{-2mm} 
\label{sec:tcompletion}
We will show the case when the tensor data is simply decimated randomly or down sampled in this section. Specifically we consider the problem of data completion from missing entries for multilinear signals.  Suppose there is an unknown tensor $\T{M}$ of size $n_1 \times n_2 \times n_3$ which is {\bf \emph{assumed to have a low tubal-rank}} and we are given a subset of entries $ \{ \T{M}_{ijk}:(i,j,k) \in \bold{\Omega} \}$ where $\bold{\Omega}$ is an indicator tensor of size $n_1 \times n_2 \times n_3$. Our objective is to recover the entire $\T{M}$. This section develops an algorithm for addressing this problem via solving the following complexity penalized algorithm:
\begin{equation}
\begin{aligned}
\label{eq:originalTNN}
\mbox{min} \hspace{4mm}&\|\T{X}\|_{TNN} \\
\mbox{subject to } \,\,\,&P_{\bold{\Omega}} ( \T{X} ) = P_{\bold{\Omega}} ( \T{M} )
\end{aligned}
\end{equation}
\noindent where $P_\bold{\Omega}$ is the orthogonal projector onto the span of tensors vanishing outside of $\bold{\Omega}$. So the $(i,j,k)_{th}$ component of $ P_{\bold{\Omega}} ( \T{X} )$ is equal to $\T{M}_{ijk}$ if $(i,j,k) \in \bold{\Omega}$ and zero otherwise. Let $\T{Y}$ be the available (sampled) data: $\T{Y} = P_\bold{\Omega} \T{M}$. Define $\mathcal{G}=\mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1}$ where $\mathscr{F}_3$ and $\mathscr{F}^{-1}_3$ are the operators representing the Fourier and inverse Fourier transform along the third dimension of tensors. Then we have
$\hat{\T{Y}} = \mathcal{G} (\hat{\T{M}})$ where $\hat{\T{Y}}$ and $\hat{\T{M}}$ are the Fourier transforms of $\T{Y}$ and $\T{M}$ along the third mode.
%In the original domain, the incomplete data is a sampling of $\T{M}$ and the sampling tensor is $P_\bold{\Omega}$. In other words, let $\T{Y}$ be the available (sampled) data, then $\T{Y} = P_\bold{\Omega} \T{M}$. Take the Fourier transform along the third dimension to the both sides we get $\hat{\T{Y}} = \mathscr{F}_3 (P_\bold{\Omega} \T{M})$, where $\mathscr{F}$ is the operator representing the Fourier transform along the third dimension of tensors. Let $\mathscr{F}^{-1}_3$ be the inverse Fourier transform along the third dimension and $\hat{\T{M}}$ be the tensor after taking Fourier transform along the third dimension of $\T{M}$. So the equation becomes $\hat{\T{Y}} = \mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1} (\hat{\T{M}})$. 
So (\ref{eq:originalTNN}) is equivalent with the following:
\begin{equation}
\begin{aligned}
\label{eq:fourierdomain_min}
\mbox{min} \hspace{4mm}&||\mbox{blkdiag}(\hat{\T{X}}) ||_*\\
\mbox{subject to } \,\,\,\,\,&\hat{\T{Y}} = {\cal G}(\hat{\T{X}}) 
\end{aligned}
\end{equation}
where $\hat{\T{X}}$ is the Fourier transform of $\T{X}$ along the third dimension and $\text{blkdiag}(\hat{\T{X}})$ is defined in (\ref{eq:blkdiag}). Noting that $\|\T{X}\|_{TNN} = ||\text{blkdiag}(\hat{\T{X}}) ||_*$. To solve the optimization problem, one can re-write (\ref{eq:fourierdomain_min}) equivalently as follows: 
\begin{equation}
\begin{aligned}
\min \hspace{4mm}& ||\text{blkdiag}( \hat{\T{Z}} )||_* + \mathbf{1}_{\hat{\T{Y}} = {\cal G}(\hat{\T{X}})} \\
\mbox{subject to } \,\,\,\,\, &\hat{\T{X}} - \hat{\T{Z}} = 0  
\end{aligned}
\end{equation}
where $\mathbf{1}$ denotes the indicator function. Then using the general framework of Alternating Direction Method of Multipliers(ADMM)\cite{Boyd_ADMM} we have the following recursion, 
\begin{align}
\label{eq:proj}
& \T{X}^{k+1} \nonumber \\
&= \arg\min_{\T{X}} \left\{ \mathbf{1}_{\T{Y} = P_{\Omega}(\T{X})} + \T{X}(:)\Tra \T{Q}^k(:)  + \frac{1}{2} || \T{X} - \T{Z}^{k}||_{F}^{2} \right\}\nonumber \\
& = \arg\min_{ \T{X}: \T{Y} = P_\Omega(\T{X}) } \left\{|| \T{X} - (\T{Z}^{k} - \T{Q}^{k})||_{F}^{2} \right\}\\
\label{eq:shrink}
& \hat{\T{Z}}^{k+1}  \nonumber \\
&= \arg \min_{\hat{\T{Z}}} \left\{ \frac{1}{\rho} ||\text{blkdiag}(\hat{\T{Z}})||_* + \frac{1}{2} ||  \hat{\T{Z}} - (\hat{\T{X}}^{k+1} + \hat{\T{Q}}^{k})||_{F}^{2} \right\}\\
& \T{Q}^{k+1} = \T{Q}^{k} + \left(\T{X}^{k+1} - \T{Z}^{k+1}\right)
\end{align}
where Equation~(\ref{eq:proj}) is least-squares projection onto the constraint and the solution to Equation~(\ref{eq:shrink}) is given by the singular value thresholding\cite{Watson92,Cai_SVT}. The $\T{X}(:)$ and $\T{Q}^k(:)$ means vectorizing the tensors which is Matlab notation.

\textbf{Equivalence of the algorithm to \emph{iterative singular-tubal shrinkage via convolution}}:
According to the particular format that (\ref{eq:shrink}) has, we can break it up into $n_3$ independent minimization problems. Let $\hat{\T{Z}}^{k+1,(i)}$ denotes the $i_{th}$ frontal slice of $\hat{\T{Z}}^{k+1}$. Similarly define $\hat{\T{X}}^{k+1,(i)}$ and $\hat{\T{Q}}^{k,(i)}$. Then (\ref{eq:shrink}) can be separated as:
\begin{equation}
\begin{aligned}
\label{eq:shrink2}
&\hat{\T{Z}}^{k+1,(i)}   \\
& = \arg \min_{W} \left\{ \frac{1}{\rho} ||W||_* + \frac{1}{2} ||  W - (\hat{\T{X}}^{k+1,(i)} + \hat{\T{Q}}^{k,(i)})||_{F}^{2} \right\}
\end{aligned}
\end{equation}
for $i = 1,2,...,n_3$. This means each $i_{th}$ frontal slice of $\hat{\T{Z}}^{k+1}$ can be calculated through (\ref{eq:shrink2}). The solution to (\ref{eq:shrink2}) can be found in\cite{Watson92,Cai_SVT,Lewis95theconvex}. In detail, if $U S V^\text{T} = (\hat{\T{X}}^{k+1,(i)} + \hat{\T{Q}}^{k,(i)})$ is the SVD of $(\hat{\T{X}}^{k+1,(i)} + \hat{\T{Q}}^{k,(i)})$, then the solution to (\ref{eq:shrink2}) is $U D_\tau (S) V^\text{T}$, where $D_\tau (S) = \text{diag}(S_{i,i} - \tau)_+$ for some positive constant $\tau$ and $``+"$ means keeping the positive part. This is equivalent to multiplying $(1-\frac{\tau}{S_{i,i}})_+$ to the $i_{th}$ singular value of $S$. So each frontal slice of $\hat{\T{Z}}^{k+1}$ can be calculated using this shrinkage on each frontal slice of $(\hat{\T{X}}^{k+1} + \hat{\T{Q}}^{k})$. Let  $\T{U} * \T{S}* \T{V}^\text{T} = (\T{X}^{k+1} + \T{Q}^{k})$ be the t-SVD of $(\T{X}^{k+1} + \T{Q}^{k})$ and $\hat{\T{S}}$ be the Fourier transform of $\T{S}$ along the third dimension. Then each element of the singular tubes of $\hat{\T{Z}}^{k+1}$ is the result of multiplying every entry $\hat{\T{S}}(i,i,j)$ with $(1-\frac{\tau}{\hat{\T{S}}(i,i,j)})_+$ for some $\tau > 0$. Since this process is carried out in the Fourier domain, in the original domain it is equivalent to convolving each tube $\T{S}(i,i,:)$ of $\T{S}$ with a real valued tubal vector $\vec{\tau}_i$ which is the inverse Fourier transform of the vector $[ ( 1-\frac{\tau_{i}(1)}{\hat{\T{S}}(i,i,1)})_+ , ( 1-\frac{\tau_{i}(2)}{\hat{\T{S}}(i,i,2)})_+ , ... , ( 1-\frac{\tau_{i}(n_3)}{\hat{\T{S}}(i,i,n_3)})_+ ]$. This operation can be captured by $\T{S}*\T{T}$, where $\T{T}$ is an f-diagonal tensor with $i_{th}$ diagonal tube to be $\vec{\tau}_i$. Then  $\T{Z}^{k+1} = \T{U}* ( \T{S}*\T{T} )* \T{V}^\text{T}$. In summary, the shrinkage operation in the Fourier domain on the singular values of each of the frontal faces is equivalent to performing a \emph{tubal shrinkage} via convolution in the original domain.


%In the actual implementation only this step is performed in the Fourier domain while all the the other steps can be done in the original domain. If the data is positive one can enforce an additional projection onto the positive cone. We will like to further remark on the shrinkage operation. It can be shown that the shrinkage operation in the Fourier domain on the singular values of each of the faces is equivalent to performing a \emph{tubal shrinkage} via convolution. 




==> rPCA__Shuchin_Aeron_s_conflicted_copy_2013-10-30_.tex <==
\section{Tensor robust Principal Component Analysis}
\label{sec:rPCA}
In this section we consider a "robust principal component analysis" problem of recovering a low tensor-multi rank tensor $\T{L}$ from a corrupted observation tensor. Similarly to the matrix robust PCA case\cite{DBLP:journals/corr/abs-0912-3599}\cite{Wright09robustprincipal}, suppose we have a third-order tensor $\T{M}$ such that it can be decomposed as
\begin{equation}
\T{M} = \T{L}_0 + \T{S}_0
\end{equation} 

\noindent where $\T{L}_0$ has low tensor-multi-rank and $\T{S}_0$ is sparse tensor. Here we focus on a case where the sparse tensor $S_0$ is tubewise sparse as shown in Figure \ref{fig:rpca1}. To resolve the low rank and the sparse components given the observation $\T{L}$ we consider the following optimization problem.

\begin{equation}
\begin{aligned}
\mbox{min} \hspace{2mm}&\|\T{L}\|_{TNN} + \lambda \|\T{S}\|_{1,1,2}\\
\mbox{subject to} \hspace{2mm}&\T{M} = \T{L} + \T{S}
\end{aligned}
\label{eq:tensor_PCA}
\end{equation}

\noindent where $\lambda>0$ and the $\|\T{S}\|_{1,1,2}$ for 3-D tensors is defined as $\sum_{i,j} ||\T{S}(i,j,:)||_{F}$. Such tensor robust PCA can be regarded as an extension of the matrix robust PCA since if the third dimension of the tensor is equal to 1.
An application where this is useful arises in multilinear imaging scenarios where some pixels can be dead/saturated or have heavy noise on them and the task is to automatically locate such pixels and recover the video. Although this may be done by processing each frame but if the noise artifacts and video features are aligned, one needs to both detect the noise and etimate the corrupted video feature.

In order to the convex optimization problem of Equation~(\ref{eq:tensor_PCA}) we use framework of ADMM. The augmented Lagrangian with the penalty term $\rho > 0$ of the problem is
\begin{equation}
\mathscr{L}_p = \|\T{L}\|_{TNN} + \lambda \|\T{S}\|_1 + \langle \T{Y} , \T{L} + \T{S} - \T{M} \rangle + \frac{\rho}{2}\|\T{L} + \T{S} - \T{M}\|_F^2
\end{equation}
\noindent where $\T{Y}$ is the dual variable and the inner product between third-order tensors is defined as (). Then we have the following recursion,
\begin{align}
\label{eq:low_rank}
&\T{L}^{k+1}=\arg\min_{\T{L}} \|\T{L}\|_{TNN} + \frac{\rho}{2} \|\T{L} + \T{S}^k - \T{M} + \T{W}^k \|^2_F\\
\label{eq:sparse}
&\T{S}^{k+1}=\arg\min_{\T{S}} \lambda \|\T{S}\|_{1,1,2} + \frac{\rho}{2} \|\T{L}^{k+1} + \T{S} - \T{M} + \T{W}^k \|^2_F\\ 
\label{eq:dual}
&\T{W}^{k+1} = \T{W}^k + \T{L}^{k+1} + \T{S}^{k+1} - \T{M}
\end{align}
\noindent where $\T{W} = \rho \T{Y}$. From section \ref{sec:tcompletion} we already have the solution to (\ref{eq:low_rank}) if we transform this equation into the Fourier domain then the tensor-nuclear-norm of $\T{L}$ will be the nuclear norm of $\text{blkdiag}(\hat{\T{L}})$. The closed form soltuion to Equation~(\ref{eq:sparse}) is given by,
\begin{equation}
\label{eq:sparse2}
\T{S}^{k+1}(i,j,:)= (1-\frac{\lambda}{\|S^k(i,j,:)\|_F})_+ \times S^k(i,j,:)
\end{equation}
\noindent where $i = 1,2,...,n_3$.

%Using the proximal gradient framework we have the following recursion:

%\begin{align}
%\label{eq:rPCA_alg}
%& \T{L}^{k+1} \nonumber \\
%& =\arg\min_{\T{L}} \|\T{L} - ( \hat{\T{L}}^k - \frac{1}{4} \bigtriangledown_{\T{L}} \|\T{M} - \T{L} - \T{S}\|_F |_{ \hat{\T{L}}^k , \hat{\T{S}}^k }  ) \|^2_F \nonumber \\
%&\hspace{5mm} + \mu \|\T{L}\|_{TNN}\\
%\nonumber \\
%& \T{S}^{k+1} \nonumber \\
%&=\arg\min_{\T{S}} \|\T{S} - ( \hat{\T{S}}^k - \frac{1}{4} \bigtriangledown_{\T{S}} \|\T{M} - \T{L} - \T{S}\|_F |_{ \hat{\T{L}}^k , \hat{\T{S}}^k }  ) \|^2_F \nonumber \\
%&\hspace{5mm} + \mu \|\T{S}\|_{1}
%\label{eq:rPCA}
%\end{align}
%
%\noindent where $(\hat{\T{L}}^k,\hat{\T{S}}^k)$ are particular chosen to achieve the higher convergence rate. See the following algorthm for detailed procedure.

%\begin{algorithm}
%\label{alg:rPCA}
%  \caption{Tensor RPCA via Proximal Gradient Method}
%  \begin{algorithmic}
%  \STATE \textbf{Input: } data tensor $\T{M} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$
%  \STATE $t_0,t_{-1} = 0$, $\mu_0 = \|\T{M}\|_F$, $\hat{\mu} = \frac{1}{10^5}\mu_0$
%  \STATE $\T{L}^{-1} , \T{L}^{0} , \T{S}^{-1}, \T{S}^{0} = 0$,
%  \STATE $\T{I} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$ \text{is the identity tensor.}
%  \STATE $\T{A} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$ \text{is the the tensor of ones.}
%  \WHILE{\text{Not Converge}}
%   \STATE $\hat{\T{L}}^k = \T{L}^k + \frac{t_{k-1}-1}{t_k} (\T{L}^k - \T{L}^{k-1})$
%   \STATE $\hat{\T{S}}^k = \T{S}^k + \frac{t_{k-1}-1}{t_k} (\T{S}^k - \T{S}^{k-1})$
%   \STATE $\T{W}^k_{\T{L}} = \hat{\T{L}}^k - \frac{1}{2}(\hat{\T{L}}^k + \hat{\T{S}}^k - \T{M}) $ 
%   \STATE $(\T{U}, \T{K}, \T{V}) = \text{tSVD}(\T{W}^k_{\T{L}})$
%   \STATE $\T{L}^{k+1} = \T{U} (\T{K} - \frac{\mu}{2} \T{I}) \T{V}^T$
%   \STATE $\T{W}^k_{\T{S}} = \hat{\T{S}}^k - \frac{1}{2}(\hat{\T{L}}^k + \hat{\T{S}}^k - \T{M}) $ 
%   \STATE $\T{S}^{k+1} = \text{sign}(\T{W}^k_{\T{S}}) * (| \T{W}^k_{\T{S}} | - \frac{\lambda \mu}{2} \T{A} )_+$
%   \STATE $t_{k+1} = \frac{-1 + \sqrt{1+4t_k^2}}{2}$
%   \STATE $\mu = \text{max}(0.9\mu,\hat{\mu})$
%  \ENDWHILE
%  \end{algorithmic}
%\end{algorithm}

%We have two experiments which use this tensor robust PCA algorithm. The first one is backgroud modeling, which is to seperate the moving object from a fixed background in a video data. In the case of background modeling, it is reasonable to assume the background is lowr-rank in traditional matrix robust PCA approach. Similarly in our experiment we assume the background is low multi-rank as a third-order tensor. So the video is the summation of a low multi-rank third-order tensor(background) and a sparse third-order tensor(object representing the activity). Figure~\ref{fig:rpca} shows the result of video with a car moving from left to right hand side. The size of each frame is $54 \times 96$, and total $38$ frames are used in the experiment.



%\begin{figure}[htbp]
%\centering \makebox[0in]{
%    \begin{tabular}{c c c}
%      \includegraphics[width = .16\textwidth]{figs/rPCA/original.png}      
%      \includegraphics[width = .16\textwidth]{figs/rPCA/lowrank.png}
%      \includegraphics[width = .16\textwidth]{figs/rPCA/sparse.png}  \\
%      
%      \includegraphics[width = .16\textwidth]{figs/rPCA/original2.png}      
%      \includegraphics[width = .16\textwidth]{figs/rPCA/lowrank2.png}
%      \includegraphics[width = .16\textwidth]{figs/rPCA/sparse2.png} 
%            
%      
%      \end{tabular}}
%  \caption{ tensor robust PCA results on background modeling. \textbf{Left}: Original video. \textbf{Middle}: Low multi-rank tensor, which is the fixed background. \textbf{Right}: Sparse tensor, which is the moving object. \textbf{First Row}: 25th frame. \textbf{Second Row}: 33th frame.  }.
%\label{fig:rpca}
%\end{figure}


For experiment we consider a video, which is compressible in the t-SVD. We randomly corrupt video data by saturating some pixels(which we call``dead pixels") with heavy additive noise. We want to estimate the locations of dead pixels using tensor robust PCA. The video used in this application is the basketball video with randomly chosen sparse dead pixels tubes along the third dimension.For each dead pixel we add gaussian noise on it. Figure~(\ref{fig:rpca1}) shows the original video and the dead pixels with noise.


\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c}
      \includegraphics[width = .24\textwidth]{figs/rPCA/video1.png}      
      \includegraphics[width = .24\textwidth]{figs/rPCA/tubal_noise.png}      
      \end{tabular}}
  \caption{ Original video and the tubal noise \textbf{Left}: Original video. \textbf{Right}: Tubal noise tensor which is sparse.}.
\label{fig:rpca1}
\end{figure}


 The size of each frame is $72 \times 128$ and the total number of frames is 80. The result is Figure~\ref{fig:rpca2}. From the results we can see that tensor robust PCA works very well on seperating the dead pixels from the video. Note that if we use the matrix robust PCA on the matricized version of this video, then the seperation will be the fixed background which is low rank, and the moving people together with the noise as the sparse part. Here we recover the video as the correct background and separate the sparse part out. 

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c c}
      \includegraphics[width = .16\textwidth]{figs/rPCA/Xn_10.png}      
      \includegraphics[width = .16\textwidth]{figs/rPCA/L_10.png}
      \includegraphics[width = .16\textwidth]{figs/rPCA/S_10.png}  \\
      
      \includegraphics[width = .16\textwidth]{figs/rPCA/Xn_20.png}      
      \includegraphics[width = .16\textwidth]{figs/rPCA/L_20.png}
      \includegraphics[width = .16\textwidth]{figs/rPCA/S_20.png} 
            
      
      \end{tabular}}
  \caption{ tensor robust PCA results on dead pixels problem. \textbf{Left}: Noisy video. \textbf{Middle}: Low rank reconstruction \textbf{Right}: Sparse reconstruction \textbf{First Row}: 40th frame. \textbf{Second Row}: 50th frame.  }.
\label{fig:rpca2}
\end{figure}


